Integrative Modeling and Analysis of the Interplay Between Epidemic and News Propagation Processes

The COVID-19 pandemic has witnessed the role of online social networks (OSNs) in the spread of infectious diseases. The rise in severity of the epidemic augments the need for proper guidelines, but also promotes the propagation of fake news-items. The popularity of a news-item can reshape the public health behaviors and affect the epidemic processes. There is a clear inter-dependency between the epidemic process and the spreading of news-items. This work creates an integrative framework to understand the interplay. We first develop a population-dependent `saturated branching process' to continually track the propagation of trending news-items on OSNs. A two-time scale dynamical system is obtained by integrating the news-propagation model with SIRS epidemic model, to analyze the holistic system. It is observed that a pattern of periodic infections emerges under a linear behavioral influence, which explains the waves of infection and reinfection that we have experienced in the pandemic. We use numerical experiments to corroborate the results and use Twitter and COVID-19 data-sets to recreate the historical infection curve using the integrative model.

==> Intro.tex <==
\section{Introduction}




Fake news becomes increasingly prevalent with the rise of online social networks (OSNs) \cite{benkler2018network,kapsikar2020controlling}. It is often generated for marketing or political purposes by social bots to manipulate public opinions and decisions. The phenomenon of confirmation bias has shown that people tend to choose news or join an online community that is consistent with their preexisting views \cite{modgil2021confirmation}. Fake news has catered to this need, and we have witnessed many cases of rapid trending of fake news in recent years. Its impact has gone beyond the influence on opinions and affected the behaviors of the people. COVID-19 is an example of this outcome;  for example during the pandemic, the fake news regarding vaccination spreads widely among social networks and causes an adverse effect on the prevention and mitigation of COVID-19 infection. Further, the deterioration of the pandemic (as COVID-19 cases increased) has in turn accelerated the creation and
propagation of fake news-items. 

%as the pandemic deteriorated of the has in turn accelerated the creating and propagation of fake news-items. %The growing number of COVID-19 cases has created public panic, which further promotes the creation and spreading of fake news. %Fake news creators can take advantage of the public panic and create misinformation to promote their agenda. For example, sellers can promote their products by misleading people to believe that they can prevent or cure COVID-19, which will cause more severe infection.

Thus the spreading of fake news and the epidemic processes are interdependent.  
%The inter-dependency can exacerbate the epidemics and accelerate the promotion of fake news. 
Hence, there is a need to understand the interplay between the two processes. There are several works discussing the relationship between information and epidemic propagation, including \cite{granell2014competing,liu2022herd,huang2022game,zhu2022preface}. They have focused on the impact of  decisions and awareness on the propagation of epidemics, assuming that individuals  take the same preventive measures once they receive the disease-related information. Very few works have explicitly modeled the dynamics of news propagation to scrutinize its inter-dependency with the spreading of infectious diseases. % news spreadig works do not explicitly model the mechanisms of the news spreading o% Even though several works have discussed the impact of two competing ideas on the propagation of epidemics, they did not consider the impact of fake news on epidemics.

The authentic news generated by appropriate authorities also plays a large role in this context.  Both types of news-items can reshape the behaviors of the population (e.g., the practice of social distancing, the decisions on vaccinations, and the compliance with mask-wearing mandates), and   can influence the growth rate of the infection. As already mentioned, this in turn can accelerate fake-news propagation. 
Thus we propose an integrative model to capture and study the interplay between the propagation of trending news-items (fake/authentic) and the epidemics (see Figure \ref{fig:my_label1}). 
%Our aim is to provide a quantitative understanding of the dynamic impact of the interplay. %fake news on the infection processes and vice versa. 
%We consider an OSN (e.g., Twitter or Facebook) during an epidemic. As depicted in Fig. \ref{fig:my_label1}., multiple news-items related to the epidemic can propagate simultaneously on the OSN. The news-items can reshape the behaviors of the population (e.g., the practice of social distancing, the decisions on vaccinations, and the compliance with mask-wearing mandates), and they can influence the growth rate of the infection. The severity of the epidemic can promote the creation and spread of fake unverified information on OSNs. 

    \begin{figure}[htbp]
           \centering
           \includegraphics[width=0.4 \textwidth]{introduction.png}
           \caption{Interplay between OSNs and epidemic networks: News spreading on OSN influences the human behavioral responses to the epidemic. The severity of the epidemic promotes the spreading of news items.}
            \label{fig:my_label1}
    \end{figure}


We first create population-dependent branching processes with saturation to model the propagation of news items on OSN and their replacement by newer topics. 
This part is inspired by the latest work on total-population-size-dependent branching processes considered in \cite{agarwal2021new,agarwal2022new,agarwal2021co}.
The epidemics-related posts on OSNs can either get viral (i.e., a large number of their copies are shared) or become extinct. A news item stops trending when its propagation saturates (i.e., it is no longer forwarded), or is replaced by another news item on the same topic. We use  stochastic approximation based approach to create a macroscopic spreading model to capture the dynamic life cycles of fake news. Second, we use a SIRS compartmental model to study the spreading of infectious diseases. The infection rate depends on the population behavior which can be strongly affected by the news propagation. We consolidate the news propagation model into the SIRS model to create an integrative framework that captures their mutual influences. We create a two-timescale dynamic process in which the fake news spreads faster than the epidemics, which is justified by the fact that online news item evolves at a much faster rate than physical human contacts. 
Furthermore, the slower process, in this case, depends upon the evolution of the faster process over a window of time, which calls for a slightly different type of two-time-scale process. 
The two-time-scale consolidated framework describes how fake news propagation can reinforce the spreading of epidemics without interventions. %epidemicWe explicitly capture the impact of the epidemics on the forwarding process using  
We analyze the dynamical system properties of the coupled system under different behavioral influences by the news content. In particular, we observe that a pattern of periodic infections emerges under a linear behavioral influence, arising from the existence of limit cycles of the dynamical system. It explains the waves of infection and reinfection that we have experienced in the pandemic. We use Twitter and COVID-19 datasets to validate the proposed model. We successfully recreate the historical infection curve by fitting and identifying the timing of news influences across the 2-year period of the COVID infection. 

\noindent{\it Organization} 
%The rest of this work is organized as follows. 
In section \ref{subsec_CP}, we introduce the OSN content propagation model, while  SIR model  is considered in section \ref{subsec_epidemic}. In section \ref{sec:interplay}, we discuss the interplay between the two and analyze the dynamical system under different behavioral patterns, while, section \ref{sec_numerical},  presents numerical results.
%The paper is concluded in Section \ref{sec:Conclusions}.




%When a post reaches a large audience, it creates more influence on the population. similarly when the epidemic is ravaging,   the panic can lead to a surge in the propagation of the related content. One can have fake-news-items further confusing the public or one can have authentic information from responsible authorities providing appropriate guidelines (which   helps to control the spread of disease). 

 

%Related works on the branching process propagation of news already exist. For example, Ralf van der Lanset al. in \cite{} have presented a detailed analysis of branching dynamics of viral information spreading. Very few works have discussed the saturation characteristic of news propagation which is important for analyzing the feature of news item update. %This work cre a saturated total-population dependent branching process to model the news propagation and couple it with spreading of epidemics for better understanding the impact of fake news propagation on epidemics evolving.


==> sim.tex <==
 
\section{Numerical Experiments}
\label{sec_numerical}




In this section, we demonstrate the ODE approximation and elaborate on the interplay between the epidemic and news propagation using the IBIN scenario. Next, we analyze the relationship between news and epidemic by imitating the realistic trajectory of COVID-19 infection level and infection rate. Finally, we learn the percentage of fake news related to COVID-19 from Twitter datasets using a BERT-based approach \cite{devlin2018bert} to corroborate the results on the interplay between fake news and the epidemic.
\subsection{ODE Approximation of News Propagation}
We first use a numerical experiment to demonstrate the ODE approximation of the stochastic iterative update (\ref{Eqn_update_stocahstic}) using (\ref{Eqn_update_ODE}). Let ${\cal M} (\theta) = \eta(i)( 1 - a \theta)$, where $\eta(i) = \bar\eta(p i + q )$, and $i$ is a constant. %To make all news items have the probability to get viral when $i$ is 1, the expected offspring ${\cal M} (\theta) = \eta(1)( 1 - a \theta)$ should be greater than 1. So here we 
Set $\bar\eta = 10$, $p = 0.9, q = 0.2, i = 1, a = 1.2, \delta_{\psi} = 0.05,   \delta_{\theta} = 0.1.$ In this experiment, we plot the sampled trajectory of (\ref{Eqn_update_stocahstic})  and its associated ODE trajectory \eqref{Eqn_update_ODE} in Fig. \ref{ODE and stochastic trajectories}. The variance of the error between the two trajectories
%stochastic trajectory 
is significantly small. 

%We also try to set the $\eta$ from 1 to 20 based on current setting to see the variance between ODE and stochastic trajectory. Figure\ref{ODE Approximation with diff eta} shows that the variance is bound to $10^{-6}$ order of magnitude which infers to a good approximation.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.39]{ODE Approximation of News Propagation1.png}
    \caption{Mean-field ODE and stochastic trajectories of news propagation}
    \label{ODE and stochastic trajectories}\vspace{-5mm}
\end{figure}

%\begin{figure}[htbp]
%\centering 
%\subfigure[The ODE and stochastic trajectory of News Propagation]{
%\label{ODE and stochastic trajectories}
%\includegraphics[width=4.2cm,height = 3.5cm]{ODE Approximation of News Propagation1.png}}
%\subfigure[The variance between ODE and stochastic trajectory with different $\eta_{k}$]{
%\label{ODE Approximation with diff eta}
%\includegraphics[width=4.2cm,height = 3.5cm]{ODE Approximation with diff eta.png}}
%\caption{ODE Approximation of News Propagation}
%\label{ODE Approximation of News Propagation}
%\end{figure}


\subsection{Interplay between Epidemics and News Propagation}
We illustrate the interplay between news and epidemic propagation. Let $\eta(i)$ take the form of $\bar\eta(pi+q)$ and $w$ be a constant in the scenario of I3N. We assume that there is a kind of fake news with influence factor $w = 0.5$. 
The lifespan of news items is much shorter than that of epidemic, and hence we update the live copies and total copies of news item every $0.00001$ time unit and update the infected fraction $i(t)$ and recovered fraction $r(t)$ every $0.005$ time unit. Let $\bar\eta = 10, p = 0.9, q = -0.1,  a = 2.5, \delta_{\psi} = 0.05, \delta_{\theta} = 0.1, p_{r} = 0.03, l_{i} = 0.00001.$
Fig. \ref{interplay_mechanism} shows four phenomena of the interplay of the I3N scenario.
\begin{itemize}
    \item[(i)] \textit{The increase in the infection level leads to the trending of news items. In turn, the treading of fake news promotes the infection level.} From Fig. \ref{interplay_mechanism_fake}, we can see that the peak values of normalized live copies $\psi(t)$ and normalized total copies $\theta(t)$ increase significantly (i.e., the news item starts trending) when  $i(t)$ reaches a relatively high value of $0.3$ indicated in  Fig. \ref{interplay_mechanism_fake}. In turn, the viral spreading of fake news promotes the propagation of the epidemic and increases the infection.
    
    \item[(ii)] \textit{News propagation affects the peak value of the epidemic.} Compared with the uncoupled SIR model, we observe that the infection level of the I3N scenario with fake news is higher than that of the uncoupled SIR model. It indicates that fake news propagation promotes epidemic spreading. 
    
    \item[(iii)] \textit{When the infection level decreases, the peak values of normalized total  and live copies decrease following the change of the corresponding limit values, $\frac{\bar\eta\left ( p i+q\right )} {a\bar\eta \left ( pi+q\right )+1}$ (see \eqref{limit_of_frac}).} Due to the property of SIR models, the infection level decreases after it reaches its peak value. One can observe that the peak values of the total and live copies also decrease after peak infection.
    %s with the infection level.
    %{\bf WHAT DO WE MEAN BY THRESHOLD HERE?}
    \item[(iv)] \textit{If the epidemic has a low infection rate or high recovery rate, then the misinformation does not have a significant impact on the epidemics, and there is no need for intervention at the early stage.} Fig. \ref{interplay_mechanism_authentic} shows that the infection level starts at $0.7$ with a lot of fake news already propagating in the online social network. %{\bf WHAT DOES IT MEAN? with the propagating fake news.} 
     Even though fake news has  a high influence factor, the infection level decreases to zero due to the high recovery rate and low infection rate. The decreased infection level leads to the vanishing of fake news, and hence it does not have a significant impact on the epidemics.% these news won't have a obvious influence on the epidemic. 
    
\begin{figure}[htbp]
    \centering \vspace{-4mm}
    \subfigure[Interplay   with a low recovery rate and a high infection rate where $i(0)$ = .001, $\bar\beta$ = .5, $\alpha$ = .2.]{
    \label{interplay_mechanism_fake}
    \includegraphics[scale=0.25]{Interplay_mechanism_fake_news1.png}}
    \vspace{0.02cm}
    \subfigure[Interplay   with a high recovery rate and a low infection rate where $i(0)$ = .7, $\bar\beta$ = .2, $\alpha$ = .5.]{
    \label{interplay_mechanism_authentic}
    \includegraphics[scale=0.41]{Interplay_mechanism_authentic_news1.png}}
    \caption{Interplay  between  fake news items and epidemic propagation in I3N.}
    \label{interplay_mechanism}\vspace{-5mm}
\end{figure}
    

\end{itemize}

%\subsection{Comparison of Epidemic Propagation Models}
%\begin{itemize}
%    \item Uncoupled SIR model with constant infection rate $\beta = 0.4$.
%    \item SIR model with increased interest towards content where $\eta(i)= 10(0.9i+0.2)$ and $w = 0.3$.
%    \item SIR model with increased influence of content where $\eta = 10$ and $w(i) = 0.3i$.
%    \item SIR model with both w(i) as well as η(i) influenced linearly where $\eta = 10(0.9i+0.2)$ and $w(i) = 0.3i$.
%\end{itemize}

%\subsection{Overall Performance}
%We analyze the performance of the four epidemic propagation models among the same time interval by comparing the infection level $i(t)$ and infection rate $r(t)$. Fig. \ref{comparison} shows that the "Increased Interest towards Content" model has the highest limit of $i(t)$ and $r(t)$ and the pure SIR model has the lowest limit of them. It is worth notice that the "Increased Influence of Content" model and "Both Interest and Influence are affected linearly" model share the same performance. 
%\begin{figure}[htbp]
%    \centering
%    \includegraphics[width=7cm,height = 3.5cm]{Compare_model.png}
%    \caption{Comparison of three different models}
%    \label{comparison}
%\end{figure}


\subsection{Validation Using Historical COVID-19 Datasets}
In this subsection, we utilize the historical Twitter and infection datasets of COVID-19 to validate the relationships between the news and epidemic propagation. 
First, we use the I3N scenario to mimic the trajectory of  COVID-19 infection level from Jan. 1, 2020 to March 15, 2022. We inject authentic or fake news items with different influence factors at discrete times and obtain the trajectory of influence factor. Let $\bar\eta = 10$, $p = 0.7, q = 0.2,  a = 1.2$,  $\bar\beta = 0.0002, \alpha = 0.0001, i(0) = 0.00001, p_{r} = 0.2, l_{i} = 0.01.$  Fig. \ref{imitation figure} shows that we successfully imitate the historical infection level. Fig. \ref{imitated influence factor} illustrates the influence factors of the news injected at different time. 

From Fig. \ref{imitation figure}, we observe that the COVID-19 epidemic propagates with a slow start from Jan. 15, 2020, to March 10, 2020. Then, COVID-19 bursts, and the infection level increases faster. It spawns a large amount of epidemic-related news. Due to the abrupt spreading of the epidemic and the nature of the panic-stricken population, many news items are fake and produce a significant influence on the epidemic during the period from March 10, 2020, to May 1, 2020, in Fig. \ref{imitated influence factor}. Once the infection level increases to a notable level, the public health agencies make efforts to spread authentic news, including advertising the precautionary measures and reporting the epidemic situation. The authentic news helps reduce the growth rate of the epidemic and produces a negative influence factor on the epidemic. The competition between fake and authentic news lasts for multiple cycles, shown in the time range from May 1, 2020, to Jan. 10, 2021, in Fig. \ref{imitated influence factor}. After the authentic news dominates for the period from Jan. 10, 2021, to Nov. 10, 2021, in Fig. \ref{imitated influence factor}, the public becomes accustomed to the epidemic and ignores the protective measures, rekindling the wide propagation of the epidemic and further producing more fake news in the following period from Nov. 10, 2021, to Jan. 1, 2022. 

\begin{figure}[htbp]
\centering 
\subfigure[Historical and fitted infection levels]{
\label{imitation figure}
\includegraphics[width=4.2cm,height = 3.5cm]{Imitated_Infection _ratio.png}}\subfigure[Influence factor by fitting]{
\label{imitated influence factor}
\includegraphics[width=4.2cm,height = 3.5cm]{Imitated_influence_factor.png}}
\caption{Fitting of the historical epidemic infection datasets}
\label{ODE Approximation of News Propagation}
\end{figure}

We analyze the COVID-related Twitter datasets from Sept. 1, 2020, to Feb. 1, 2021, and obtain the percentage of fake news using a BERT-based approach to corroborate the results on the interplay between the epidemic and fake news. Since we pick a long time interval of $6$ months with the significant change in historical infection rate, it's hard to analyze all daily Twitter datasets. So we just pick those at the beginning of each month to show the tendency of the percentage of fake news.  Fig. \ref{fig:fake_news_ratio} shows that the percentage of fake news on Twitter is positively correlated with the historical infection rate. The red stars indicate the percentage of fake news on
Twitter at discrete time points. The blue line shows the historical infection rate. When the epidemic becomes severer, it generates public panic and promotes the spreading of fake news. Hence, the percentage of fake news on Twitter increases. However, when the epidemic becomes less aggressive, the percentage of fake news decreases.
\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.4]{fake_news_ratio.png}
    \caption{Relationship between the historical infection rate and the percentage of fake news on Twitter. Red stars indicate the percentage of fake news on Twitter and the blue line shows the historical infection rate.}
    \label{fig:fake_news_ratio}\vspace{-3mm}
\end{figure}

 




